Assessing the Feasibility of Web-Request Prediction Models on Mobile Platforms

Prefetching web pages is a well-studied solution to reduce network latency by predicting users' future actions based on their past behaviors. However, such techniques are largely unexplored on mobile platforms. Today's privacy regulations make it infeasible to explore prefetching with the usual strategy of amassing large amounts of data over long periods and constructing conventional, "large" prediction models. Our work is based on the observation that this may not be necessary: Given previously reported mobile-device usage trends (e.g., repetitive behaviors in brief bursts), we hypothesized that prefetching should work effectively with "small" models trained on mobile-user requests collected during much shorter time periods. To test this hypothesis, we constructed a framework for automatically assessing prediction models, and used it to conduct an extensive empirical study based on over 15 million HTTP requests collected from nearly 11,500 mobile users during a 24-hour period, resulting in over 7 million models. Our results demonstrate the feasibility of prefetching with small models on mobile platforms, directly motivating future work in this area. We further introduce several strategies for improving prediction models while reducing the model size. Finally, our framework provides the foundation for future explorations of effective prediction models across a range of usage scenarios.

==> related.tex <==
\section{Related Work}
\label{sec:related}

Web prefetching is a fundamental research area and has attracted a large body of work for decades~\cite{de2007web,de2010referrer,davison2002predicting,gunduz2003web,ruamviboonsuk2017vroom,mickens2010crom,wang2016speeding,choi2018appx,zhao2018leveraging,wang2012far,palpanas1998webppm,padmanabhan1996usingDG,ibrahim2000neural,pitkow1999mininglongestrepeatin,ban2007online,yang2004building}.
Over the recent years, prefetching techniques have been identified as promising in the emerging mobile computing domain~\cite{higgins2012informed, zhao2018empirically}, and have become a crowded area, including the work on identifying performance bottlenecks~\cite{nejati2016depth,wang2013demystifying,vesuna2016caching}, balancing trade-offs between prefetching benefits and waste~\cite{higgins2012informed,ruxton2008time}, and identifying ``what'' and ``when'' to prefetch~\cite{zhao2018empirically, zhao2018leveraging, choi2018appx, mickens2010crom,wang2016speeding}. 
As discussed earlier, our study specifically focuses on evaluating the accuracy of history-based prefetching techniques based on different prediction models for mobile platforms.

A large body of work leverages historical data to decide ``what'' and ``when'' to prefetch on the proxy- or server-side~\cite{agababov2015flywheel,butkiewicz2015klotski,rosen2017push,ruamviboonsuk2017vroom}.
In our work, we focus on applying prediction models on the client-side based on individual users, thus is complementary to existing work.
EarlyBird \cite{wang2015earlybird} and PocketWeb \cite{lymberopoulos2012pocketweb} studied mobile user's historical data to prefetch web content, but they are only applicable to their specific domain, such as Twitter.
Cachekeeper~\cite{zhang2013cachekeeper} studied the redundant requests to identify caching opportunities, but did not analyze the sequence of historical requests like our work.
Wang et al. ~\cite{wang2012far} explored \emph{most-popular} (MP) prediction algorithm on 24 mobile users' historical requests collected for over a year.
However, our study focuses on a fine-grained analysis to explore the lower bound of the suitable data size to train the prediction models based on a significantly larger user base as discussed in Section~\ref{sec:intro}.
